ASAP-MPC: An Asynchronous Update Scheme for Online Motion Planning with Nonlinear Model Predictive Control

This paper presents a Nonlinear Model Predictive Control (NMPC) scheme targeted at motion planning for mechatronic motion systems, such as drones and mobile platforms. NMPC-based motion planning typically requires low computation times to be able to provide control inputs at the required rate for system stability, disturbance rejection, and overall performance. Although there exist various ways in literature to reduce the solution times in NMPC, such times may not be low enough to allow real-time implementations. This paper presents ASAP-MPC, an approach to handle varying, sometimes restrictively large, solution times with an asynchronous update scheme, always allowing for full convergence and real-time execution. The NMPC algorithm is combined with a linear state feedback controller tracking the optimised trajectories for improved robustness against possible disturbances and plant-model mismatch. ASAP-MPC seamlessly merges trajectories, resulting from subsequent NMPC solutions, providing a smooth and continuous overall trajectory for the motion system. This frameworks applicability to embedded applications is shown on two different experiment setups where a state-of-the-art method fails: a quadcopter flying through a cluttered environment in hardware-in-the-loop simulation and a scale model truck-trailer manoeuvring in a structured lab environment.

==> commented_parts.tex <==
% trajectory optimization for (optimal) motion planning is a strongly researched field, as it is a powerful strategy to deploy autonomous robot manipulators, ground robots and aerial robots. Nonlinear Model Predictive Control (NMPC) is one of the more popular strategies to implement/achieve online, optimal motion planning. It allows users to deploy a (physics-based) model of their system and specify constraints such as actuator limits, obstacle avoidance, etc. to which any NMPC solution will adhere. \\



% Broad lit study
% RHP: bergman 2020, Ljungqvist 2019
% Non-NMPC: Pivtoraiko 2013
% Sampling-based: Frazzoli, Hsu

% % MPC lit study - fixed
% Zavala aNMPC
% Obayashi MPC + feedback
% NMPC: CIAO Diehl, STORM Dieter Fox
% Feedback MPC: Grandia et al. (IROS 2019, feedback MPC legged robots)


% Possible references
% References: Mellinger and Kumar (2011) ?, CIAO paper Diehl, Neunert, % GusTO, 
% (Shiller Z, Sharma S, Stern I, Stern A (2013) On-line obstacle avoidance at high speed), Bai Li 2021 (autonomous parking), Adajania (ICRA 2023, AMSwarm paper)
% Handig boek: Motion and Operation Planning of Robotic Systems, Giuseppe Carbone; fernando gomez-bravo
% \red{references blabla} show Nonlinear Model Predictive Control (NMPC) applied to drones (die van de EDFs bv), self-driving cars, ...


% Non-NMPC references:  Ljungqvist, %Campos-Macías (RAL 2017, hybrid motion planning), 
% Deep RL: Shuai Li (2022)

% In a classical MPC scheme, an optimal control problem (OCP) is solved in every time step, at the full control rate that is required to (1) stabilize the motion system, (2) agilely control it, (3) reject disturbances acting on it or (4) safely react to environmental changes \red{[ref]}. Furthermore, it assumes that the solution to the OCP is instantaneously available. However, any NMPC implementation always involves a (significant) finite computation time. Guaranteeing a feasible, locally optimal solution at the full control rate is a challenging task, especially for applications that involve nonlinear systems, long planning horizons, complex environments, or limited onboard computation power. 
%A high research effort is spent on developing fast algorithms to solve the OCP within the short available time. %, exploiting the specific structure of the OCP, or ... \red{[ref to solvers and stuff]}.

% {\color{red} Add general literature study on some MPC examples}
